Drug Recommendation toward Safe Polypharmacy

Adverse drug reactions (ADRs) induced from high-order drug-drug interactions (DDIs) due to polypharmacy represent a significant public health problem. In this paper, we formally formulate the to-avoid and safe (with respect to ADRs) drug recommendation problems when multiple drugs have been taken simultaneously. We develop a joint model with a recommendation component and an ADR label prediction component to recommend for a prescription a set of to-avoid drugs that will induce ADRs if taken together with the prescription. We also develop real drug-drug interaction datasets and corresponding evaluation protocols. Our experimental results on real datasets demonstrate the strong performance of the joint model compared to other baseline methods.

==> figure/convergence/plot_convergence.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3456.00,1728.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(213,172){\makebox(0,0)[r]{\strut{}\footnotesize 1.1}}%
      \put(213,398){\makebox(0,0)[r]{\strut{}\footnotesize 1.3}}%
      \put(213,624){\makebox(0,0)[r]{\strut{}\footnotesize 1.5}}%
      \put(213,850){\makebox(0,0)[r]{\strut{}\footnotesize 1.7}}%
      \put(213,1075){\makebox(0,0)[r]{\strut{}\footnotesize 1.9}}%
      \put(213,1301){\makebox(0,0)[r]{\strut{}\footnotesize 2.1}}%
      \put(213,1527){\makebox(0,0)[r]{\strut{}\footnotesize 2.3}}%
      \put(389,-48){\makebox(0,0){\strut{}\footnotesize 1}}%
      \put(719,-48){\makebox(0,0){\strut{}\footnotesize 10}}%
      \put(1085,-48){\makebox(0,0){\strut{}\footnotesize 20}}%
      \put(1451,-48){\makebox(0,0){\strut{}\footnotesize 30}}%
      \put(1817,-48){\makebox(0,0){\strut{}\footnotesize 40}}%
      \put(2183,-48){\makebox(0,0){\strut{}\footnotesize 50}}%
      \put(2550,-48){\makebox(0,0){\strut{}\footnotesize 60}}%
      \put(2916,-48){\makebox(0,0){\strut{}\footnotesize 70}}%
      \put(3282,-48){\makebox(0,0){\strut{}\footnotesize 80}}%
      \put(352,1719){\makebox(0,0)[l]{\strut{}\footnotesize $\times 10^{4}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-161,906){\rotatebox{-270}{\makebox(0,0){\strut{}objective function $L$}}}%
      \put(1813,-268){\makebox(0,0){\strut{}ADMM iterations}}%
      \csname LTb\endcsname%
      \put(2295,1467){\makebox(0,0)[r]{\strut{}$\modelIn$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_convergence}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> table/accuracy_top10.tex <==
        &        \multirow{2}{*}{\modelIn} &     \predScr	& 0.2467 & 0.2467 & 0.3110 \\
        &                                  &     \predBin	& 0.2467 & 0.2467 & 0.3110 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.2286 & 0.2284 & 0.2926 \\
        &                                  &     \predBin 	& 0.2286 & 0.2284 & 0.2926 \\
        &                            \Rand &            - 	& 0.0073 & 0.0148 & 0.0279 \\
        &                          \LROnly &            - 	& 0.2239 & 0.2241 & 0.2928 \\
        &                        \SLIMOnly &            - 	& 0.2273 & 0.2271 & 0.2968 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\
        &        \multirow{2}{*}{\modelIn} &     \predScr 	& 0.3434 & 0.3432 & 0.3439 \\
        &                                  &     \predBin 	& 0.3434 & 0.3432 & 0.3439 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.3234 & 0.3238 & 0.3327 \\
        &                                  &     \predBin 	& 0.3234 & 0.3238 & 0.3327 \\
        &                            \Rand &            - 	& 0.0051 & 0.0103 & 0.0051 \\
        &                          \LROnly &            - 	& 0.2391 & 0.2391 & 0.1515 \\
        &                        \SLIMOnly &            - 	& 0.3240 & 0.3238 & 0.3419 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\
        &        \multirow{2}{*}{\modelIn} &     \predScr	& 0.2467 & 0.2467 & 0.3110 \\
        &                                  &     \predBin	& 0.2467 & 0.2467 & 0.3110 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.2286 & 0.2284 & 0.2926 \\
        &                                  &     \predBin 	& 0.2286 & 0.2284 & 0.2926 \\
        &                            \Rand &            - 	& 0.0073 & 0.0148 & 0.0279 \\
        &                          \LROnly &            - 	& 0.2239 & 0.2241 & 0.2928 \\
        &                        \SLIMOnly &            - 	& 0.2273 & 0.2271 & 0.2968 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\
        &        \multirow{2}{*}{\modelIn} &     \predScr 	& 0.3434 & 0.3432 & 0.3439 \\
        &                                  &     \predBin 	& 0.3434 & 0.3432 & 0.3439 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.3234 & 0.3238 & 0.3327 \\
        &                                  &     \predBin 	& 0.3234 & 0.3238 & 0.3327 \\
        &                            \Rand &            - 	& 0.0051 & 0.0103 & 0.0051 \\
        &                          \LROnly &            - 	& 0.2391 & 0.2391 & 0.1515 \\
        &                        \SLIMOnly &            - 	& 0.3240 & 0.3238 & 0.3419 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\


==> table/accuracy_top20.tex <==
        &        \multirow{2}{*}{\modelIn} &     \predScr	& 0.2694 & 0.2695 & 0.3289 \\
        &                                  &     \predBin	& 0.2694 & 0.2695 & 0.3289 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.2477 & 0.2476 & 0.2956 \\
        &                                  &     \predBin 	& 0.2478 & 0.2476 & 0.2956 \\
        &                            \Rand &            - 	& 0.0108 & 0.0215 & 0.0341 \\
        &                          \LROnly &            - 	& 0.2530 & 0.2530 & 0.3287 \\
        &                        \SLIMOnly &            - 	& 0.2723 & 0.2722 & 0.3045 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\
        &        \multirow{2}{*}{\modelIn} &     \predScr 	& 0.4265 & 0.4273 & 0.4135 \\
        &                                  &     \predBin 	& 0.4265 & 0.4273 & 0.4135 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.4051 & 0.4049 & 0.3996 \\
        &                                  &     \predBin 	& 0.4051 & 0.4049 & 0.3996 \\
        &                            \Rand &            - 	& 0.0099 & 0.0201 & 0.0099 \\
        &                          \LROnly &            - 	& 0.3158 & 0.3154 & 0.2107 \\
        &                        \SLIMOnly &            - 	& 0.3975 & 0.3982 & 0.4175 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\


==> table/max_metrics.tex <==
\begin{table}[h!]
\vspace{-0mm}
  \centering
  \caption{Maximum of Evaluation Metrics}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule


	\DataPoll			&\recall   &  \precision  & \accuracy  \\
	%\hline
	\midrule								
		\Dall  			& 0.3516        & 0.4925        & 0.5831 \\
		\Dataset		& 0.9404        & 0.1690        & 0.1783 \\

        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'' and ``acc'' represent recall, precision, and accuracy, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table}
%


==> table/max_metrics_Neg.tex <==
\begin{table}[h!]
\vspace{-0mm}
  \centering
  \caption{Maximum of Evaluation Metrics Negative Label}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule


	\DataPoll			 & \recall   &  \precision  & \accuracy  \\
	%\hline
	\midrule								
		\Dall  			 & 0.0549	& 0.6738	& 0.5831\\
		\Dataset		 & 0.8394	& 0.1876	& 0.1783\\


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'' and ``acc'' represent recall, precision, and accuracy, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table}
%


==> table/max_metrics_Neg_Top10.tex <==
\begin{table}[h!]
\vspace{-0mm}
  \centering
  \caption{Maximum of Evaluation Metrics Negative Label Top-$10$}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule


	\DataPoll			 & \recall   &  \precision  & \accuracy  \\
	%\hline
	\midrule								
		\Dall  		 & 0.1028	& 0.6305	& 0.5013\\
		\Dataset	 & 0.9657	& 0.1079	& 0.0977\\






        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'' and ``acc'' represent recall, precision, and accuracy, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table}
%


==> table/max_metrics_Neg_Top20.tex <==
\begin{table}[h!]
\vspace{-0mm}
  \centering
  \caption{Maximum of Evaluation Metrics Negative Label Top-$20$}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule


	\DataPoll			 & \recall   &  \precision  & \accuracy  \\
	%\hline
	\midrule								
		\Dall  			& 0.1869	& 0.5732	& 0.4168 \\
		\Dataset		& 0.9984	& 0.0558	& 0.0503 \\






        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'' and ``acc'' represent recall, precision, and accuracy, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table}
%


==> table/max_metrics_Top10.tex <==
\begin{table}[h!]
\vspace{-0mm}
  \centering
  \caption{Maximum of Evaluation Metrics Top-$10$}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule


	\DataPoll			&\recall   &  \precision  & \accuracy  \\
	%\hline
	\midrule								
		\Dall  		& 0.5311	& 0.3721	& 0.5013\\
		\Dataset	& 0.9731	& 0.0874	& 0.0977\\





        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'' and ``acc'' represent recall, precision, and accuracy, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table}
%


==> table/max_metrics_Top20.tex <==
\begin{table}[h!]
\vspace{-0mm}
  \centering
  \caption{Maximum of Evaluation Metrics Top-$20$}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule


	\DataPoll			&\recall   &  \precision  & \accuracy  \\
	%\hline
	\midrule								
		\Dall  			& 0.7436	& 0.2605	& 0.4168\\
		\Dataset		& 0.9955	& 0.0447	& 0.0503\\








        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'' and ``acc'' represent recall, precision, and accuracy, respectively.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table}
%


==> table/notation_table.tex <==
\begin{table}[h]
  \caption{Table of Notations}
  \label{tbl:Notation}
  \centering
  \begin{threeparttable}
%  \renewcommand\arraystretch{1.2}
    \begin{small}
      \begin{tabular}{
	@{\hspace{2pt}}l@{\hspace{10pt}}
	@{\hspace{2pt}}p{0.77\linewidth}@{\hspace{ 2pt}}
	}
        %\hline\hline
	\toprule
	    {Notation}					& Description	\\
		\midrule
%		{\drug}					& Drug\\
		{\D}					& a prescription\\
		{\Dset}					& a set of prescriptions \\
%		{\A}								 & Binary drug combination matrix \\
%		$\boldsymbol{a}_{i}^{\intercal}$     & Binary drug combination vector for $\D_i$ \\
		\SLIMLogR				& Learning $W$, $x$ and $c$ jointly \\
		\Rand					& Random recommendation and prediction \\
		\LROnly				& Recommendation based on top-5 prediction scores\\
		\SLIMOnly				& Recommendation only\\
		\Sep					& Separate model for Recommendation and Prediction\\
        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
		  ~~
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
  \end{threeparttable}
%\vspace{-5mm}
\end{table}
%
 


==> table/old_file/performance_recall_Rec_20.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Recall Rec 20}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & rec   & pre   & acc & avg& pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline
	\midrule								
						
				
\multirow{ 8}{*}{ \Dall } 	 	
			  	
			  	
			  	
		          	& $\SLIMLogRWepInScr 	$      	&0.1252 &0.1754 &0.3065 &0.2024 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-2,-4)$\\
			 	& $\SLIMLogRWepInBin 	$      	&0.1252 &0.1754 &0.3066 &0.2024 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-2,-4)$\\
				& $\SLIMLogRWepExScr 	$ 	&0.1387 &0.1943 &0.2728 &0.2019 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-6,-6)$\\
				& $\SLIMLogRWepExBin 	$ 	&0.1185 &0.1659 &0.2310 &0.1718 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-6,-6)$\\
			  	& \Rand  			&0.0026 &0.0072 &0.0151 &0.0083 &$(--,--,--,--,--)$\\		
     			  	& \LROnly	        	&0.1098 &0.1538 &0.1768 &0.1468 &$(--,--,--,-4,-2)$\\		
			  	& \SLIMOnly			&0.1127 &0.1579 &0.2970 &0.1892 &$(--,-\infty,~~1,--,--)$\\	
			  	& \Sep       			&0.1149 &0.1609 &0.2949 &0.1902 &$(--,-4,~~0,-2,~~0)$\\		


	
	
	
	



	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				
				
				& $\SLIMLogRWepInScr 	$	&0.5808 &0.1044 &0.1877 &0.2910 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-2,-4)$\\
				& $\SLIMLogRWepInBin 	$	&0.5808 &0.1044 &0.1877 &0.2910 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-2,-4)$\\
				& $\SLIMLogRWepExScr 	$	&0.7985 &0.1434 &0.1668 &0.3696 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-6,-6)$\\
				& $\SLIMLogRWepExBin 	$       &0.6204 &0.1114 &0.1282 &0.2867 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-6,-6)$\\
				& \Rand  			&0.0065 &0.0023 &0.0018 &0.0035 &$(--,--,--,--,--)$\\	
				& \LROnly	                &0.4516 &0.0811 &0.0532 &0.1953 &$(--,--,--,-4,-2)$\\	
				& \SLIMOnly			&0.5404 &0.0971 &0.1852 &0.2742 &$(--,-5,~~0,--,--)$\\	
				&\Sep           		&0.5494 &0.0987 &0.1833 &0.2771 &$(--,-3,~~0,-2,~~0)$\\	


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'', ``acc'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/parameter_study_accuracy.tex <==
\begin{table}[h!]
\vspace{-0mm}
  \centering
  \caption{\accuracy of \modelIn with \predScr (top-5)}
  \label{table:param:accuracy}
  \begin{threeparttable}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}|
	  @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
         %
        }
	\toprule
	{$\omega\backslash\alpha$}& {100} &  {50} &  {20} &  {10} &  {5} \\ %& 1 \\
	\midrule								
	100    & 0.2809 & 0.2677 & 0.2646 & 0.2562 & 0.2612 \\%& 0.2890 \\			
	50     & 0.2869 & 0.2831 & 0.2794 & 0.2672 & 0.2732 \\%& 0.2907 \\     
	20     & 0.2951 & 0.2919 & 0.2890 & 0.2895 & 0.2874 \\%& 0.2888 \\                    
	10     & 0.2943 & 0.2967 & 0.2938 & 0.2915 & 0.2891 \\%& 0.2874 \\    
	5      & 0.2955 & 0.2969 & 0.2958 & 0.2951 & 0.2924 \\%& 0.2898 \\      
	1      & 0.2938 & 0.2953 & 0.2936 & 0.2919 & 0.2893 \\% & 0.2878 \\			
	\bottomrule
      \end{tabular}
%      \begin{tablenotes}
%        \setlength\labelsep{0pt}
%	\begin{footnotesize}
%	\item
%	\mbox{}
%	\par
%	\end{footnotesize}
%      \end{tablenotes}
  \end{threeparttable}
\end{table}
%


==> table/parameter_study_precision.tex <==
\begin{table}[h!]
  \centering
  \caption{\precision of \modelIn with \predScr (top-5)}
  \label{table:param:precision}
  \begin{threeparttable}
%   \begin{center}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}|
	  @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
        }
	\toprule
        {$\omega\backslash\alpha$}& {100} &  {50} &  {20} &  {10} &  {5} \\ %& 1 \\
        %\backslashbox{$\omega$}{$\alpha$}	        & 100 & 50 & 20 & 10 & 5 & 1 \\
	%\hline
	\midrule								
	100		& 0.2298 & 0.2311 & 0.2282 & 0.2264 & 0.2254 \\%& 0.2268 \\	
	50              & 0.2315 & 0.2335 & 0.2339 & 0.2325 & 0.2254 \\%& 0.2294 \\        
	20              & 0.2325 & 0.2343 & 0.2347 & 0.2349 & 0.2339 \\%& 0.2313 \\        
	10              & 0.2315 & 0.2351 & 0.2351 & 0.2359 & 0.2345 \\%& 0.2319 \\        
	5               & 0.2321 & 0.2355 & 0.2361 & 0.2359 & 0.2341 \\%& 0.2317 \\          
	1		& 0.2315 & 0.2327 & 0.2321 & 0.2305 & 0.2290 \\%& 0.2288 \\        
	\bottomrule
      \end{tabular}
%      \begin{tablenotes}
%        \setlength\labelsep{0pt}
%	\begin{footnotesize}
%	\item
%	\mbox{}
%	\par
%	\end{footnotesize}
%      \end{tablenotes}
  \end{threeparttable}
\end{table}
%


==> table/parameter_study_recall.tex <==
\begin{table}[h!]
\vspace{-0mm}
  \centering
  \caption{\recall of \modelIn with \predScr (top-5)}
  \label{table:param:recall}
  \begin{threeparttable}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}|
	  @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
          @{\hspace{3pt}}r@{\hspace{3pt}}
%	  @{\hspace{3pt}}r@{\hspace{3pt}}
         %
        }
	\toprule
	%
	%\backslashbox{$\omega$}{$\alpha$}
        %        \textcolor{white}{$\omega$}{$\alpha$}& \multirow{2}{*}{100} &  \multirow{2}{*}{50} &  \multirow{2}{*}{20} &  \multirow{2}{*}{10} &  \multirow{2}{*}{5} \\ %& 1 \\
        {$\omega\backslash\alpha$}& {100} &  {50} &  {20} &  {10} &  {5} \\ %& 1 \\
%        $\omega$\textcolor{white}{$\alpha$} & & & & & \\
	\midrule								
	100		& 0.2298 & 0.2309 & 0.2281 & 0.2264 & 0.2255 \\%& 0.2270 \\	
	50              & 0.2315 & 0.2335 & 0.2341 & 0.2324 & 0.2255 \\%& 0.2295 \\        
	20              & 0.2324 & 0.2344 & 0.2346 & 0.2349 & 0.2338 \\%& 0.2312 \\        
	10              & 0.2315 & 0.2352 & 0.2349 & 0.2358 & 0.2344 \\%& 0.2318 \\        
	5               & 0.2318 & 0.2355 & 0.2361 & 0.2361 & 0.2341 \\%& 0.2315 \\        	
	1		& 0.2315 & 0.2327 & 0.2321 & 0.2304 & 0.2290 \\%& 0.2287 \\	
	\bottomrule
      \end{tabular}
%      \begin{tablenotes}
%        \setlength\labelsep{0pt}
%	\begin{footnotesize}
%	\item
%	\mbox{}
%	\par
%	\end{footnotesize}
%      \end{tablenotes}
  \end{threeparttable}
\end{table}
%


==> table/performance_accuracy.ibk.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Accuracy}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
    
    
    
    
    
    
    
    

	
	\DataPoll	&\multicolumn{1}{l}{Method} & rec   & pre   & acc & avg& pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline
	\midrule								
%\rowcolor{gray!50}											
\multirow{ 12}{*}{ \Dall } 	
				&  $\modelInScr          $  	&0.0173 &0.1652 &0.4120 &0.1982 &$(-1,-1,~~1,-3,-8)$\\
%\rowcolor{gray!50}	  	
				&  $\modelInBin          $      &0.0516 &0.2070 &0.4294 &0.2293 &$(~~2,-2,~~0,-6,-8)$\\
%\rowcolor{gray!50}	  	
				&  $\modelExScr          $      &0.0589 &0.1960 &0.3987 &0.2179 &$(-1,-\infty,~~1,-4,-8)$\\
%\rowcolor{gray!50}	  	
				&  $\modelExBin          $      &0.0298 &0.1778 &0.3923 &0.2000 &$(-2,-\infty,~~0,-4,-4)$\\
%\rowcolor{gray!50}              
				&  $\SLIMLogRWepInScr    $      &0.0216 &0.1992 &0.4618 &0.2275 &$(~~0,-2,-2,-6,-6,~~1,~~1,-4,-6)$\\
%\rowcolor{gray!50}              
				&  $\SLIMLogRWepInBin    $      &0.0668 &0.2129 &0.5140 &0.2646 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-2,-6)$\\
%\rowcolor{gray!50}	  	
				&  $\SLIMLogRWepExScr    $	&0.0825 &0.1857 &0.5279 &0.2654 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-2,-6)$\\
%\rowcolor{gray!50}	  	
				&  $\SLIMLogRWepExBin    $	&0.0952 &0.1812 &0.4771 &0.2512 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-2,-6)$\\
			  	&   \Rand  			&0.0026 &0.0072 &0.0289 &0.0129 &$(--,--,--,--,--)$\\      	
     			  	&   \LROnly	        	&0.0013 &0.0019 &0.0019 &0.0017 &$(--,--,--,-4,~~6)$\\     	
			  	&   \SLIMOnly			&0.1127 &0.1579 &0.2970 &0.1892 &$(--,-\infty,~~1,--,--)$\\	
			  	&   \Sep		    	&0.0730 &0.2011 &0.4132 &0.2291 &$(--,-6,~~1,-5,-\infty)$\\  	

	%\hline
	\midrule

%\rowcolor{gray!50}
\multirow{ 12}{*}{ \Dataset }	
				&  $\modelInScr          $	&0.0953 &0.1260 &0.2289 &0.1501 &$(-1,-3,-1,-3,-\infty)$\\		
%\rowcolor{gray!50}	 	
				&  $\modelInBin          $	&0.3802 &0.1474 &0.2646 &0.2641 &$(-1,-4,~~1,-6,-8)$\\			
%\rowcolor{gray!50}		
				&  $\modelExScr          $	&0.3676 &0.1310 &0.2438 &0.2475 &$(-1,-4,~~0,-\infty,-\infty)$\\	
%\rowcolor{gray!50}		
				&  $\modelExBin          $	&0.3651 &0.1328 &0.2395 &0.2458 &$(-1,-2,~~1,-4,-8)$\\			
%\rowcolor{gray!50}              
				&  $\SLIMLogRWepInScr    $	&0.1167 &0.1497 &0.2940 &0.1868 &$(~~0,-2,-2,-8,-8,~~0,~~0,-4,-6)$\\
%\rowcolor{gray!50}              
				&  $\SLIMLogRWepInBin    $	&0.3100 &0.1342 &0.3268 &0.2570 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-2,-6)$\\
%\rowcolor{gray!50}              
				&  $\SLIMLogRWepExScr    $	&0.4467 &0.1290 &0.3369 &0.3042 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-2,-6)$\\
%\rowcolor{gray!50}              
				&  $\SLIMLogRWepExBin    $	&0.4941 &0.1207 &0.3191 &0.3113 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-2,-6)$\\		   
				&   \Rand  			&0.0065 &0.0023 &0.0024 &0.0037 &$(--,--,--,--,--)$\\            	
				&   \LROnly	        	&0.0083 &0.0015 &0.0016 &0.0038 &$(--,--,--,-3,-1)$\\                    
				&   \SLIMOnly			&0.5377 &0.0966 &0.1852 &0.2732 &$(--,-2,-2,--,--)$\\            	
				&   \Sep		        &0.3955 &0.1393 &0.2643 &0.2664 &$(--,-4,~~1,-\infty,-\infty)$\\         

        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'', ``acc'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_accuracy.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Accuracy}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule


	\DataPoll	&\multicolumn{1}{l}{Method} & rec   & pre   & acc & avg& pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline
	\midrule								
\multirow{ 12}{*}{ \Dall } 	
				&  $\modelInScr          $  &0.0168 &0.1626 &0.4124 &0.1973 &$(-1,-2,~~1,-3,-8)$\\
				&  $\modelInBin          $  &0.0516 &0.2070 &0.4294 &0.2293 &$(~~2,-2,~~0,-6,-8)$\\
				&  $\modelExScr          $  &0.0589 &0.1960 &0.3987 &0.2179 &$(-1,-\infty,~~1,-4,-8)$\\
				&  $\modelExBin          $  &0.0298 &0.1778 &0.3923 &0.2000 &$(-2,-\infty,~~0,-4,-4)$\\
				&  $\SLIMLogRWepInScr    $  &0.0216 &0.1992 &0.2309 &0.1506 &$(~~0,-2,-2,-6,-6,~~1,~~1,-4,-6)$\\
				&  $\SLIMLogRWepInBin    $  &0.0668 &0.2129 &0.2570 &0.1789 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-2,-6)$\\
				&  $\SLIMLogRWepExScr    $  &0.0825 &0.1857 &0.2640 &0.1774 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-2,-6)$\\
				&  $\SLIMLogRWepExBin    $  &0.0952 &0.1812 &0.2386 &0.1717 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-2,-6)$\\
			  	&   \Rand  			&0.0026 &0.0072 &0.0151 &0.0083 &$(--,--,--,--,--)$\\
     			  	&   \LROnly	        	&0.0011 &0.0015 &0.0012 &0.0013 &$(--,--,--,-6,-4)$\\
			  	&   \SLIMOnly			&0.1127 &0.1579 &0.2970 &0.1892 &$(--,-\infty,~~1,--,--)$\\
			  	&   \Sep		    	&0.0777 &0.2017 &0.2328 &0.1707 &$(--,-\infty,~~1,-6,-6)$\\

	%\hline
	\midrule

\multirow{ 12}{*}{ \Dataset }	
				&  $\modelInScr          $	&0.0953 &0.1260 &0.2289 &0.1501 &$(-1,-3,-1,-3,-\infty)$\\
				&  $\modelInBin          $      &0.3802 &0.1474 &0.2646 &0.2641 &$(-1,-4,~~1,-6,-8)$\\
				&  $\modelExScr          $      &0.3675 &0.1314 &0.2445 &0.2478 &$(-1,-5,~~0,-8,-\infty)$\\
				&  $\modelExBin          $      &0.3236 &0.1372 &0.2398 &0.2335 &$(-1,-\infty,~~2,-4,-9)$\\
				&  $\SLIMLogRWepInScr    $	&0.1167 &0.1497 &0.1470 &0.1378 &$(~~0,-2,-2,-8,-8,~~0,~~0,-4,-6)$\\
				&  $\SLIMLogRWepInBin    $      &0.3100 &0.1342 &0.1634 &0.2025 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-2,-6)$\\
				&  $\SLIMLogRWepExScr    $      &0.4467 &0.1290 &0.1684 &0.2480 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-2,-6)$\\
				&  $\SLIMLogRWepExBin    $      &0.4941 &0.1207 &0.1595 &0.2581 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-2,-6)$\\     
				&   \Rand  		  	&0.0065 &0.0023 &0.0018 &0.0035 &$(--,--,--,--,--)$\\
				&   \LROnly	                &0.0087 &0.0016 &0.0012 &0.0038 &$(--,--,--,-6,-4)$\\
				&   \SLIMOnly		        &0.5377 &0.0966 &0.1852 &0.2732 &$(--,-2,-2,--,--)$\\
				&   \Sep		        &0.4093 &0.1378 &0.1586 &0.2352 &$(--,-\infty,-\infty,-\infty,-\infty)$\\

        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'', ``acc'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_accuracy_Rec_20.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Accuracy}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & \recall   &  \precision  & \accuracy & avg & pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline



	\midrule								
\multirow{ 8}{*}{ \Dall } 	 	
		          	& $\SLIMLogRWepInScr 	$    &0.0817 &0.1145 &0.1708 &0.1223 &$(~~0,-6,~~1,-2,-4)$\\
			 	& $\SLIMLogRWepInBin 	$    &0.0817 &0.1145 &0.1708 &0.1223 &$(~~0,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepExScr 	$    &0.0738 &0.1034 &0.1631 &0.1134 &$(~~0,-8,~~1,-2,-6)$\\
				& $\SLIMLogRWepExBin 	$    &0.0741 &0.1038 &0.1631 &0.1137 &$(~~0,-8,~~1,-2,-4)$\\
			  	& \Rand  		     &0.0021 &0.0058 &0.0139 &0.0073 &$(--,--,--,--,--)$\\
     			  	& \LROnly	             &0.0716 &0.1004 &0.1439 &0.1053 &$(--,--,--,-2,~~5)$\\
			  	& \SLIMOnly		     &0.0710 &0.0995 &0.1650 &0.1118 &$(--,-1,~~6,--,--)$\\
			  	& \Sep       		     &0.0710 &0.0995 &0.1647 &0.1117 &$(--,-1,~~6,-2,~~0)$\\


	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				& $\SLIMLogRWepInScr 	$	&0.2435 &0.0438 &0.0505 &0.1126 &$(~~0,-8,~~1,-2,-6)$\\
				& $\SLIMLogRWepInBin 	$	&0.2435 &0.0438 &0.0505 &0.1126 &$(~~0,-8,~~1,-2,-6)$\\
				& $\SLIMLogRWepExScr 	$	&0.2329 &0.0419 &0.0493 &0.1080 &$( -2,-8,~~1,-2,-2)$\\
				& $\SLIMLogRWepExBin 	$       &0.2329 &0.0419 &0.0493 &0.1080 &$( -2,-8,~~1,-2,-2)$\\
				& \Rand  			&0.0027 &0.0010 &0.0006 &0.0014 &$(--,--,--,--,--)$\\
				& \LROnly	                &0.1674 &0.0301 &0.0184 &0.0720 &$(--,--,--,-3,-2)$\\
				& \SLIMOnly			&0.2289 &0.0411 &0.0495 &0.1065 &$(--,-2,~~2,--,--)$\\
				&\Sep           		&0.2289 &0.0411 &0.0495 &0.1065 &$(--,-4,~~2,-2,~~0)$\\


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``\recall'', ``\precision'', ``\accuracy'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_accuracy_Rec_20Neg.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Accuracy (Neg label)}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & \recall   &  \precision  & \accuracy & avg & pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline


	\midrule								
\multirow{ 8}{*}{ \Dall } 	 	
		          	& $\SLIMLogRWepInScr 	$    &0.0185 &0.2271 &0.1708 &0.1388 &$(~~0,-6,~~1,-2,-4)$\\
			 	& $\SLIMLogRWepInBin 	$    &0.0185 &0.2270 &0.1708 &0.1388 &$(~~0,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepExScr 	$    &0.0181 &0.2224 &0.1631 &0.1345 &$(~~0,-8,~~1,-2,-4)$\\
				& $\SLIMLogRWepExBin 	$    &0.0181 &0.2224 &0.1631 &0.1345 &$(~~0,-8,~~1,-2,-4)$\\
			  	& \Rand  		 &0.0020 &0.0498 &0.0139 &0.0219 &$(--,--,--,--,--)$\\       
     			  	& \LROnly	         &0.0153 &0.1873 &0.1439 &0.1155 &$(--,--,--,-2,~~0)$\\      
			  	& \SLIMOnly		 &0.0188 &0.2304 &0.1650 &0.1381 &$(--,-1,~~6,--,--)$\\      
			  	& \Sep       		 &0.0187 &0.2300 &0.1647 &0.1378 &$(--,-1,~~6,-2,~~0)$\\     


	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				& $\SLIMLogRWepInScr 	$	&0.2546 &0.0569 &0.0505 &0.1207 &$(~~0,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepInBin 	$	&0.2546 &0.0569 &0.0505 &0.1207 &$(~~0,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepExScr 	$	&0.2535 &0.0567 &0.0493 &0.1198 &$(-2,-8,~~1,-2,-2)$\\
				& $\SLIMLogRWepExBin 	$       &0.2535 &0.0567 &0.0493 &0.1198 &$(-2,-8,~~1,-2,-2)$\\
				& \Rand  		&0.0031 &0.0014 &0.0006 &0.0017 &$(--,--,--,--,--)$\\  	
				& \LROnly	        &0.0298 &0.0067 &0.0184 &0.0183 &$(--,--,--,-3,-2)$\\          
				& \SLIMOnly		&0.2585 &0.0578 &0.0495 &0.1219 &$(--,-2,~~2,--,--)$\\ 	
				& \Sep           	&0.2585 &0.0578 &0.0495 &0.1219 &$(--,-4,~~2,-2,~~0)$\\	


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``\recall'', ``\precision'', ``\accuracy'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_accuracy_Rec_20_Top_10.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Accuracy Top-$10$}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & \recall   &  \precision  & \accuracy & avg & pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline



	\midrule								
\multirow{ 8}{*}{ \Dall } 	 	
		          	& $\SLIMLogRWepInScr 	$    &0.1310 &0.0918 &0.1559 &0.1262 &$(~~0,-6,~~1,-2,-4)$\\
			 	& $\SLIMLogRWepInBin 	$    &0.1310 &0.0918 &0.1559 &0.1262 &$(~~0,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepExScr 	$    &0.1214 &0.0850 &0.1467 &0.1177 &$(~~0,-8,~~1,-2,-4)$\\
				& $\SLIMLogRWepExBin 	$    &0.1214 &0.0850 &0.1467 &0.1177 &$(~~0,-8,~~1,-2,-4)$\\
			  	& \Rand  		     &0.0039 &0.0055 &0.0140 &0.0078 &$(--,--,--,--,--)$\\
     			  	& \LROnly	             &0.1189 &0.0834 &0.1468 &0.1164 &$(--,--,--,-3,~~0)$\\
			  	& \SLIMOnly		     &0.1207 &0.0845 &0.1488 &0.1180 &$(--,-1,~~6,--,--)$\\
			  	& \Sep       		     &       &       &       &       &       \\
















	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				& $\SLIMLogRWepInScr 	$	&0.3342 &0.0300 &0.0336 &0.1326 &$(~~0,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepInBin 	$	&0.3342 &0.0300 &0.0336 &0.1326 &$(~~0,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepExScr 	$	&0.3147 &0.0283 &0.0325 &0.1252 &$( -2,-8,~~1,-2,-4)$\\
				& $\SLIMLogRWepExBin 	$       &0.3147 &0.0283 &0.0325 &0.1252 &$( -2,-8,~~1,-2,-4)$\\
				& \Rand  			&0.0050 &0.0009 &0.0005 &0.0021 &$(--,--,--,--,--)$\\
				& \LROnly	                &0.2327 &0.0209 &0.0148 &0.0895 &$(--,--,--,-2,~~0)$\\
				& \SLIMOnly			&0.3153 &0.0283 &0.0334 &0.1257 &$(--,-5,~~2,--,--)$\\
				&\Sep           		&       &       &       &       &       \\


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``\recall'', ``\precision'', ``\accuracy'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_accuracy_Rec_20_Top_20.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Accuracy Top-$20$}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & \recall   &  \precision  & \accuracy & avg & pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline



	\midrule								
\multirow{ 8}{*}{ \Dall } 	 	
		          	& $\SLIMLogRWepInScr 	$    &0.2003 &0.0702 &0.1371 &0.1359 &$(~~1,-6,~~1,-2,-6)$\\
			 	& $\SLIMLogRWepInBin 	$    &0.2003 &0.0702 &0.1371 &0.1359 &$(~~1,-6,~~1,-2,-6)$\\
				& $\SLIMLogRWepExScr 	$    &0.1842 &0.0645 &0.1232 &0.1240 &$(~~0,-8,~~1,-2,-4)$\\
				& $\SLIMLogRWepExBin 	$    &0.1843 &0.0645 &0.1232 &0.1240 &$(~~0,-8,~~1,-2,-4)$\\
			  	& \Rand  		     &0.0080 &0.0056 &0.0142 &0.0093 &$(--,--,--,--,--)$\\
     			  	& \LROnly	             &0.1881 &0.0659 &0.1370 &0.1303 &$(--,--,--,-4,-2)$\\
			  	& \SLIMOnly		     &0.2025 &0.0709 &0.1269 &0.1334 &$(--,-1,~~6,--,--)$\\
			  	& \Sep       		     &       &       &       &       &       \\




	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				& $\SLIMLogRWepInScr 	$	&0.4246 &0.0191 &0.0208 &0.1548 &$(~~0,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepInBin 	$	&0.4246 &0.0191 &0.0208 &0.1548 &$(~~0,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepExScr 	$	&0.4033 &0.0181 &0.0201 &0.1472 &$( -2,-6,~~1,-2,-2)$\\
				& $\SLIMLogRWepExBin 	$       &0.4033 &0.0181 &0.0201 &0.1472 &$( -2,-6,~~1,-2,-2)$\\
				& \Rand  			&0.0099 &0.0009 &0.0005 &0.0038 &$(--,--,--,--,--)$\\
				& \LROnly	                &0.3144 &0.0141 &0.0106 &0.1130 &$(--,--,--,-3,~~0)$\\
				& \SLIMOnly			&0.3957 &0.0178 &0.0210 &0.1448 &$(--,-1,~~6,--,--)$\\
				&\Sep           		&       &       &       &       &       \\


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``\recall'', ``\precision'', ``\accuracy'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_accuracy_Until_5.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Accuracy Until five}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
 	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & rec   & pre   & acc & avg& pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ 
			&$\text{meanN}^{+}$  &$\text{stdN}^{+}$  &$\text{meanN}^{-}$  &$\text{stdN}^{-}$  &$\text{Rec5}{\%}$ &$\text{Rec5}{\%}$\\
	%\hline
	\midrule								

				
\multirow{ 8 }{*}{ \Dall } 	 	
		        & $\SLIMLogRWepInScr 	$ 	&0.0030 &0.0722 &0.4404 &0.1719 &$(~~0,-2,-2,-6,-6,~~0,~~0,-6,-4)$      &1151.98        &251.48 &104.64 &329.29 &0.05   &0.92\\
			& $\SLIMLogRWepInBin 	$       &0.0166 &0.1720 &0.4286 &0.2057 &$(~~0,~~1,~~1,~~0,~~0,~~1,~~1,-2,-2)$  &1125.34        &294.06 &385.01 &558.08 &0.07   &0.68\\      
			& $\SLIMLogRWepExScr 	$  	&0.0219 &0.1631 &0.4058 &0.1969 &$(~~0,-2,-2,-8,-8,~~1,~~1,-4,-6)$      &1101.89        &333.95 &103.52 &323.06 &0.09   &0.92\\
			& $\SLIMLogRWepExBin 	$  	&0.0337 &0.1384 &0.3703 &0.1808 &$(~~0,-2,-2,-8,-8,~~1,~~1,-4,-6)$      &1082.51        &360.97 &129.25 &359.82 &0.10   &0.90\\
			& \Rand  			&0.0026 &0.0072 &0.0151 &0.0083 &$(--,--,--,--,--)$\\
     			& \LROnly	        	&0.1087 &0.1613 &0.1681 &0.1460 &$(--,--,--,-6,-2)$\\
			& \SLIMOnly			&0.1127 &0.1579 &0.2970 &0.1892 &$(--,-\infty,~~1,--,--)$\\
			& \Sep      			&0.0002 &0.0460 &0.4186 &0.1549 &$(--,-1,~~3,-6,-5)$    &1200.71        &82.47  &5.00   &0.00   &0.01   &1.00\\
	%\hline
	\midrule
\multirow{ 8 }{*}{ \Dataset }	
				
				
				
				& $\SLIMLogRWepInScr 	$	&0.0225 &0.0701 &0.2782 &0.1236 &$(~~0,-2,-2,-6,-6,~~0,~~0,-6,-4)$      &1151.98        &251.48 &104.64 &329.29 &0.05   &0.92\\
				& $\SLIMLogRWepInBin 	$	&0.0851 &0.1143 &0.2723 &0.1572 &$(~~0,~~1,~~1,~~0,~~0,~~1,~~1,-2,-2)$  &1125.34        &294.06 &385.01 &558.08 &0.07   &0.68\\
				& $\SLIMLogRWepExScr 	$	&0.1097 &0.1054 &0.2562 &0.1571 &$(~~0,-2,-2,-8,-8,~~1,~~1,-4,-4)$      &1101.89        &333.95 &103.52 &323.06 &0.09   &0.92\\
				& $\SLIMLogRWepExBin 	$       &0.1456 &0.0772 &0.2326 &0.1518 &$(~~0,-2,-2,-6,-6,~~1,~~1,-4,-4)$      &1082.51        &360.97 &129.26 &359.82 &0.10   &0.90\\
				& \Rand  			&0.0065 &0.0023 &0.0018 &0.0035 &$(--,--,--,--,--)$\\
				& \LROnly	                &0.4494 &0.0854 &0.0846 &0.2065 &$(--,--,--,-5,-2)$\\
				& \SLIMOnly			&0.5377 &0.0966 &0.1852 &0.2732 &$(--,-2,-2,--,--)$\\
				& \Sep		        	&0.0440 &0.0782 &0.2649 &0.1290 &$(--,-\infty,-\infty,-3,-2)$   &1118.61        &312.53 &51.46  &227.45 &0.07   &0.96\\
		
 	

 	
 	


        %\hline\hline
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
        \begin{footnotesize}
        \item
        In this table, ``rec'', ``pre'', ``acc'' and ``pars'' represent
        recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
        \end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}        
  \end{threeparttable}
\end{table*}



==> table/performance_precision.ibk.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Precision}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & rec   & pre   & acc & avg& pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline
	\midrule								

     
     
     
     
     
     
     
     
										
\multirow{ 12}{*}{ \Dall } 	&  $\modelInScr          $	&0.0153 &0.1887 &0.3926 &0.1989 &$(-2,~~0,-2,-4,-8)$\\            	 	
			  	&  $\modelInBin          $	&0.0366 &0.2447 &0.4233 &0.2349 &$(-1,-6,-3,-3,-8)$\\                    
%\rowcolor{gray!50}	  	
				&  $\modelExScr          $	&0.0945 &0.2141 &0.3605 &0.2230 &$(~~0,-10,~~1,-9,-8)$\\                 
			  	&  $\modelExBin          $	&0.1253 &0.2060 &0.2657 &0.1990 &$(~~1,-\infty,~~1,-\infty,-8)$\\        
%\rowcolor{gray!50}             
				&  $\SLIMLogRWepInScr    $	&0.0274 &0.2267 &0.4325 &0.2289 &$(~~0,-2,-2,~~0,~~0,~~0,~~0,-4,-6)$\\
%\rowcolor{gray!50}             
				&  $\SLIMLogRWepInBin    $	&0.0376 &0.2566 &0.4720 &0.2554 &$(~~0,-2,-2,-6,-6,~~0,~~0,-4,-6)$\\
%\rowcolor{gray!50}	  	
				&  $\SLIMLogRWepExScr    $	&0.0324 &0.1970 &0.4638 &0.2311 &$(~~0,~~0,~~0,-8,-8,-2,-2,-2,-4)$\\
%\rowcolor{gray!50}	  	
				&  $\SLIMLogRWepExBin    $	&0.1270 &0.2091 &0.3691 &0.2351 &$(~~0,~~1,~~1,-6,-6,-2,-2,-6,-6)$\\
			  	&   \Rand  	   	  	&0.0026 &0.0072 &0.0289 &0.0129 &$(--,--,--,--,--)$\\		
     			  	&   \LROnly	   	  	&0.0013 &0.0020 &0.0019 &0.0017 &$(--,--,--,-5,~~1)$\\		
			  	&   \SLIMOnly	   	  	&0.1127 &0.1579 &0.2970 &0.1892 &$(--,-\infty,~~1,--,--)$\\	
			  	&   \Sep		  	&0.0582 &0.2024 &0.3854 &0.2153 &$(--,~~0,-3,-2,-5)$\\		  	


	%\hline
	\midrule

%\rowcolor{gray!50}
\multirow{ 12}{*}{ \Dataset }	&  $\modelInScr          $	&0.1150 &0.1370 &0.2222 &0.1581 &$(-1,~~0,-1,-3,-8)$\\
%\rowcolor{gray!50}	 	
				&  $\modelInBin          $	&0.2161 &0.1841 &0.2496 &0.2166 &$(-1,-3,~~0,-3,-9)$\\
%\rowcolor{gray!50}		
				&  $\modelExScr          $	&0.5589 &0.1520 &0.1851 &0.2987 &$(~~1,-\infty,~~1,-\infty,-8)$\\
%\rowcolor{gray!50}		
				&  $\modelExBin          $	&0.7079 &0.1506 &0.1873 &0.3486 &$(~~1,-\infty,~~0,-\infty,-9)$\\
%\rowcolor{gray!50}              
				&  $\SLIMLogRWepInScr    $	&0.1502 &0.1595 &0.2685 &0.1927 &$(~~0,-2,-2,~~0,~~0,~~0,~~0,-4,-6)$\\
%\rowcolor{gray!50}              
				&  $\SLIMLogRWepInBin    $	&0.2148 &0.1884 &0.3110 &0.2381 &$(~~0,-2,-2,-6,-6,~~0,~~0,-4,-6)$\\
%\rowcolor{gray!50}              
				&  $\SLIMLogRWepExScr    $	&0.5030 &0.1422 &0.2879 &0.3110 &$(~~0,~~1,~~1,-8,-8,~~1,~~1,-4,-4)$\\
%\rowcolor{gray!50}              
				&  $\SLIMLogRWepExBin    $	&0.7504 &0.1585 &0.2609 &0.3899 &$(~~0,~~1,~~1,-6,-6,-2,-2,-6,-6)$\\     
				&   \Rand  			&0.0065 &0.0023 &0.0024 &0.0037 &$(--,--,--,--,--)$\\  	
				&   \LROnly			&0.0081 &0.0016 &0.0016 &0.0038 &$(--,--,--,-4,~~1)$\\         
				&   \SLIMOnly			&0.5402 &0.0971 &0.1852 &0.2742 &$(--,-3,~~0,--,--)$\\ 	
				&   \Sep	 		&0.3164 &0.1418 &0.2418 &0.2333 &$(--,-4,~~0,-2,-4)$\\         

        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'', ``acc'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_precision.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Precision}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & rec   & pre   & acc & avg& pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline
	\midrule								


     
\multirow{ 12}{*}{ \Dall } 	&  $\modelInScr          $	&0.0153 &0.1887 &0.3926 &0.1989 &$(-2,~~0,-2,-4,-8)$\\            	
			  	&  $\modelInBin          $	&0.0366 &0.2447 &0.4233 &0.2349 &$(-1,-6,-3,-3,-8)$\\
				&  $\modelExScr          $	&0.0945 &0.2151 &0.3611 &0.2236 &$(~~0,-3,~~1,-\infty,-8)$\\
			  	&  $\modelExBin          $	&0.1253 &0.2060 &0.2657 &0.1990 &$(~~1,-\infty,~~1,-\infty,-8)$\\
				&  $\SLIMLogRWepInScr    $	&0.0274 &0.2267 &0.2163 &0.1568 &$(~~0,-2,-2,~~0,~~0,~~0,~~0,-4,-6)$\\
				&  $\SLIMLogRWepInBin    $	&0.0376 &0.2566 &0.2360 &0.1767 &$(~~0,-2,-2,-6,-6,~~0,~~0,-4,-6)$\\
				&  $\SLIMLogRWepExScr    $	&0.0324 &0.1970 &0.2319 &0.1538 &$(~~0,~~0,~~0,-8,-8,-2,-2,-2,-4)$\\
				&  $\SLIMLogRWepExBin    $	&0.1270 &0.2091 &0.1846 &0.1736 &$(~~0,~~1,~~1,-6,-6,-2,-2,-6,-6)$\\	
			  	&   \Rand  	   	  	&0.0026 &0.0072 &0.0151 &0.0083 &$(--,--,--,--,--)$\\
     			  	&   \LROnly	   	  	&0.0013 &0.0020 &0.0012 &0.0015 &$(--,--,--,-4,~~1)$\\
			  	&   \SLIMOnly	   	  	&0.1127 &0.1579 &0.2970 &0.1892 &$(--,-\infty,~~1,--,--)$\\
			  	&   \Sep		  	&0.0624 &0.2054 &0.2161 &0.1613 &$(--,-1,~~1,-2,-5)$\\		

	%\hline
	\midrule

\multirow{ 12}{*}{ \Dataset }	&  $\modelInScr          $	&0.1150 &0.1370 &0.2222 &0.1581 &$(-1,~~0,-1,-3,-8)$\\
				&  $\modelInBin          $      &0.2161 &0.1841 &0.2496 &0.2166 &$(-1,-3,~~0,-3,-9)$\\
				&  $\modelExScr          $      &0.5589 &0.1520 &0.1851 &0.2987 &$(~~1,-\infty,~~1,-\infty,-8)$\\
				&  $\modelExBin          $      &0.7079 &0.1506 &0.1873 &0.3486 &$(~~1,-\infty,~~0,-\infty,-9)$\\
				&  $\SLIMLogRWepInScr    $	&0.1502 &0.1595 &0.1342 &0.1480 &$(~~0,-2,-2,~~0,~~0,~~0,~~0,-4,-6)$\\
				&  $\SLIMLogRWepInBin    $      &0.2148 &0.1884 &0.1555 &0.1862 &$(~~0,-2,-2,-6,-6,~~0,~~0,-4,-6)$\\
				&  $\SLIMLogRWepExScr    $      &0.5030 &0.1422 &0.1440 &0.2631 &$(~~0,~~1,~~1,-8,-8,~~1,~~1,-4,-4)$\\
				&  $\SLIMLogRWepExBin    $      &0.7504 &0.1585 &0.1305 &0.3465 &$(~~0,~~1,~~1,-6,-6,-2,-2,-6,-6)$\\	
				&   \Rand  			&0.0065 &0.0023 &0.0018 &0.0035 &$(--,--,--,--,--)$\\
				&   \LROnly			&0.0081 &0.0016 &0.0010 &0.0036 &$(--,--,--,-4,~~1)$\\
				&   \SLIMOnly			&0.5402 &0.0971 &0.1852 &0.2742 &$(--,-3,~~0,--,--)$\\
				&   \Sep	 		&0.3238 &0.1404 &0.1475 &0.2039 &$(--,-\infty,-\infty,-2,-4)$\\

        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'', ``acc'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_precision_Rec_20.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Precision}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & \recall   &  \precision  & \accuracy & avg & pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline

	\midrule								
\multirow{ 8}{*}{ \Dall } 	 	
		          	& $\SLIMLogRWepInScr 	$   &0.0829 &0.1162 &0.1700 &0.1230 &$(~~1,-6,~~1,-2,-6)$\\  
			 	& $\SLIMLogRWepInBin 	$   &0.0829 &0.1162 &0.1700 &0.1230 &$(~~1,-6,~~1,-2,-6)$\\  
				& $\SLIMLogRWepExScr 	$   &0.0741 &0.1038 &0.1630 &0.1136 &$(~~0,-6,~~1,-2,-4)$\\  
				& $\SLIMLogRWepExBin 	$   &0.0741 &0.1038 &0.1630 &0.1136 &$(~~0,-6,~~1,-2,-4)$\\  
			  	& \Rand  		    &0.0021 &0.0058 &0.0139 &0.0073 &$(--,--,--,--,--)$\\      
     			  	& \LROnly	            &0.0732 &0.1025 &0.1417 &0.1058 &$(--,--,--,-4,-2)$\\      
			  	& \SLIMOnly		    &0.0748 &0.1048 &0.1638 &0.1145 &$(--,-3,~~2,--,--)$\\     
			  	& \Sep       		    &0.0748 &0.1048 &0.1639 &0.1145 &$(--,-\infty,~~2,-2,~~0)$\\    


	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				& $\SLIMLogRWepInScr 	$	&0.2457 &0.0442 &0.0503 &0.1134 &$(~~1,-8,~~1,-2,-6)$\\
				& $\SLIMLogRWepInBin 	$	&0.2457 &0.0442 &0.0503 &0.1134 &$(~~1,-8,~~1,-2,-6)$\\
				& $\SLIMLogRWepExScr 	$	&0.2329 &0.0419 &0.0492 &0.1080 &$( -2,-6,~~1,-2,-2)$\\
				& $\SLIMLogRWepExBin 	$       &0.2329 &0.0419 &0.0492 &0.1080 &$( -2,-6,~~1,-2,-2)$\\	
				& \Rand  			&0.0027 &0.0010 &0.0006 &0.0014 &$(--,--,--,--,--)$\\
				& \LROnly	                &0.1674 &0.0301 &0.0184 &0.0720 &$(--,--,--,-3,-2)$\\
				& \SLIMOnly			&0.2318 &0.0417 &0.0491 &0.1075 &$(--,-3,~~1,--,--)$\\
				&\Sep           		&0.2318 &0.0417 &0.0491 &0.1075 &$(--,-4,~~1,-2,~~0)$\\


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``\recall'', ``\precision'', ``\accuracy'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_precision_Rec_20Neg.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Precision (Neg label)}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & \recall   &  \precision  & \accuracy & avg & pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline









	\midrule								
\multirow{ 8}{*}{ \Dall } 	 	
		          	& $\SLIMLogRWepInScr 	$   &0.0185 &0.2272 &0.1705 &0.1387 &$(~~0,-8,~~1,-2,-4)$\\
			 	& $\SLIMLogRWepInBin 	$   &0.0185 &0.2272 &0.1705 &0.1387 &$(~~0,-8,~~1,-2,-4)$\\
				& $\SLIMLogRWepExScr 	$   &0.0181 &0.2227 &0.1631 &0.1346 &$(~~0,-8,~~1,-2,-6)$\\
				& $\SLIMLogRWepExBin 	$   &0.0181 &0.2226 &0.1630 &0.1346 &$(~~0,-8,~~1,-2,-6)$\\
			  	& \Rand  		 &0.0020 &0.0498 &0.0139 &0.0219 &$(--,--,--,--,--)$\\     
     			  	& \LROnly	         &0.0153 &0.1874 &0.1439 &0.1155 &$(--,--,--,-2,~~5)$\\    
			  	& \SLIMOnly		 &0.0188 &0.2304 &0.1650 &0.1381 &$(--,-1,~~6,--,--)$\\    
			  	& \Sep       		 &0.0187 &0.2300 &0.1647 &0.1378 &$(--,-1,~~6,-2,~~0)$\\    









	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				& $\SLIMLogRWepInScr 	$	&0.2558 &0.0572 &0.0505 &0.1212 &$(~~0,-8,~~1,-2,-6)$\\
				& $\SLIMLogRWepInBin 	$	&0.2558 &0.0572 &0.0505 &0.1212 &$(~~0,-8,~~1,-2,-6)$\\
				& $\SLIMLogRWepExScr 	$	&0.2535 &0.0567 &0.0493 &0.1198 &$(-2,-8,~~1,-2,-2)$\\
				& $\SLIMLogRWepExBin 	$       &0.2535 &0.0567 &0.0493 &0.1198 &$(-2,-8,~~1,-2,-2)$\\	
				& \Rand  			&0.0031 &0.0014 &0.0006 &0.0017 &$(--,--,--,--,--)$\\
				& \LROnly	                &0.0347 &0.0078 &0.0181 &0.0202 &$(--,--,--,-2,~~5)$\\
				& \SLIMOnly			&0.2585 &0.0578 &0.0495 &0.1219 &$(--,-2,~~2,--,--)$\\
				&\Sep           		&0.2589 &0.0579 &0.0495 &0.1221 &$(--,-6,~~2,-2,~~0)$\\


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``\recall'', ``\precision'', ``\accuracy'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_precision_Rec_20_Top_10.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Precision Top-$10$}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & \recall   &  \precision  & \accuracy & avg & pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline

	\midrule								
\multirow{ 8}{*}{ \Dall } 	 	
		          	& $\SLIMLogRWepInScr 	$   &0.1326 &0.0929 &0.1542 &0.1266 &$(~~1,-6,~~1,-2,-4)$\\
			 	& $\SLIMLogRWepInBin 	$   &0.1326 &0.0929 &0.1541 &0.1265 &$(~~1,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepExScr 	$   &0.1213 &0.0850 &0.1462 &0.1175 &$(~~0,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepExBin 	$   &0.1213 &0.0850 &0.1461 &0.1175 &$(~~0,-6,~~1,-2,-4)$\\
			  	& \Rand  		    &0.0039 &0.0055 &0.0140 &0.0078 &$(--,--,--,--,--)$\\
     			  	& \LROnly	            &0.1191 &0.0835 &0.1397 &0.1141 &$(--,--,--,-5,-2)$\\
			  	& \SLIMOnly		    &0.1234 &0.0865 &0.1474 &0.1191 &$(--,-3,~~2,--,--)$\\
			  	& \Sep       		    &       &       &       &       &       \\ 


	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				& $\SLIMLogRWepInScr 	$	&0.3371 &0.0303 &0.0333 &0.1336 &$(~~1,-6,~~1,-2,-6)$\\
				& $\SLIMLogRWepInBin 	$	&0.3371 &0.0303 &0.0333 &0.1336 &$(~~1,-6,~~1,-2,-6)$\\
				& $\SLIMLogRWepExScr 	$	&0.3169 &0.0285 &0.0324 &0.1259 &$(~~0,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepExBin 	$       &0.3169 &0.0285 &0.0324 &0.1259 &$(~~0,-6,~~1,-2,-4)$\\
				& \Rand  			&0.0050 &0.0009 &0.0005 &0.0021 &$(--,--,--,--,--)$\\
				& \LROnly	                &0.2343 &0.0211 &0.0148 &0.0901 &$(--,--,--,-3,-1)$\\
				& \SLIMOnly			&0.3153 &0.0283 &0.0333 &0.1256 &$(--,-3,~~2,--,--)$\\
				&\Sep           	&       &       &       &       &       \\


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``\recall'', ``\precision'', ``\accuracy'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_precision_Rec_20_Top_20.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Precision Top-$20$}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & \recall   &  \precision  & \accuracy & avg & pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline

	\midrule								
\multirow{ 8}{*}{ \Dall } 	 	
		          	& $\SLIMLogRWepInScr 	$  &0.2145 &0.0752 &0.1151 &0.1349 &$(~~1,~~0,~~1,-2,-2)$\\ 
			 	& $\SLIMLogRWepInBin 	$  &0.2146 &0.0752 &0.1149 &0.1349 &$(~~1,~~0,~~1,-2,-2)$\\ 
				& $\SLIMLogRWepExScr 	$  &0.1881 &0.0659 &0.1193 &0.1244 &$(~~1, -6,~~1,-2,-2)$\\ 
				& $\SLIMLogRWepExBin 	$  &0.1886 &0.0661 &0.1191 &0.1246 &$(~~1, -6,~~1,-2,-2)$\\ 
			  	& \Rand  		 &0.0080 &0.0056 &0.0142 &0.0093 &$(--,--,--,--,--)$\\     
     			  	& \LROnly	         &0.1881 &0.0659 &0.1370 &0.1303 &$(--,--,--,-4,-2)$\\     
			  	& \SLIMOnly		 &0.2023 &0.0709 &0.1256 &0.1329 &$(--,~~0,~~6,--,--)$\\   
			  	& \Sep       		    &       &       &       &       &       \\ 






	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				& $\SLIMLogRWepInScr 	$	&0.4383 &0.0197 &0.0202 &0.1594 &$(~~1, -6,~~1,-2,-2)$\\
				& $\SLIMLogRWepInBin 	$	&0.4383 &0.0197 &0.0202 &0.1594 &$(~~1, -6,~~1,-2,-2)$\\
				& $\SLIMLogRWepExScr 	$	&0.4042 &0.0182 &0.0199 &0.1474 &$( -2, -8,~~1,-4,-6)$\\
				& $\SLIMLogRWepExBin 	$       &0.4042 &0.0182 &0.0199 &0.1474 &$( -2, -8,~~1,-4,-6)$\\
				& \Rand  	&0.0099 &0.0009 &0.0005 &0.0038 &$(--,--,--,--,--)$\\ 		
				& \LROnly	&0.3169 &0.0142 &0.0104 &0.1138 &$(--,--,--,-4,-2)$\\                 
				& \SLIMOnly	&0.4121 &0.0185 &0.0208 &0.1505 &$(--,-2,~~2,--,--)$\\		
				&\Sep           	&       &       &       &       &       \\


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``\recall'', ``\precision'', ``\accuracy'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_precision_Until_5.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Precision Until five}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
 	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & rec   & pre   & acc & avg& pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ 
			&$\text{meanN}^{+}$  &$\text{stdN}^{+}$  &$\text{meanN}^{-}$  &$\text{stdN}^{-}$  &$\text{Rec5}{\%}$ &$\text{Rec5}{\%}$\\
	%\hline
	\midrule								
						
				
\multirow{ 8 }{*}{ \Dall } 	 	
		        & $\SLIMLogRWepInScr 	$ 	&0.0285 &0.2039 &0.3839 &0.2054 &$(~~0,-2,-2,~~0,~~0,-2,-2,-4,-6)$      &1091.22        &354.67 &74.87  &276.17 &0.10   &0.94\\
			& $\SLIMLogRWepInBin 	$       &0.0652 &0.2134 &0.3980 &0.2255 &$(~~0,~~0,~~0,-6,-6,~~0,~~0,-2,-6)$    &1070.45        &377.65 &159.82 &401.83 &0.11   &0.87\\       
			& $\SLIMLogRWepExScr 	$  	&0.0971 &0.1932 &0.3039 &0.1981 &$(~~0,~~1,~~1,-8,-8,~~1,~~1,-6,-6)$    &552.78 &597.12 &176.56 &420.15 &0.55   &0.86\\		       
			& $\SLIMLogRWepExBin 	$  	&0.1341 &0.1881 &0.2809 &0.2010 &$(~~0,~~1,~~1,-8,-8,~~1,~~1,-6,-6)$    &17.88  &86.36  &752.73 &563.01 &1.00   &0.41\\		       
			& \Rand  			&0.0026 &0.0072 &0.0151 &0.0083 &$(--,--,--,--,--)$\\
     			& \LROnly	        	&0.1087 &0.1613 &0.1681 &0.1460 &$(--,--,--,-6,-2)$\\
			& \SLIMOnly			&0.1127 &0.1579 &0.2970 &0.1892 &$(--,-\infty,~~1,--,--)$\\
			& \Sep      			&0.0499 &0.1940 &0.3578 &0.2006 &$(--,~~0,~~0,-2,0)$    &953.42 &490.37 &147.12 &386.86 &0.21   &0.88\\

	%\hline
	\midrule
\multirow{ 8 }{*}{ \Dataset }	
				
				
				& $\SLIMLogRWepInScr 	$	&0.1553 &0.1436 &0.2380 &0.1790 &$(~~0,-2,-2,~~0,~~0,~~0,~~0,-4,-6)$    &1091.93        &353.75 &74.39  &275.41 &0.10   &0.94\\		
				& $\SLIMLogRWepInBin 	$	&0.0999 &0.1386 &0.0755 &0.1047 &$(~~0,~~1,~~1,-8,-8,-2,-2,-2,-2)$      &1139.67        &260.97 &1159.92        &227.46 &0.06   &0.04\\
				& $\SLIMLogRWepExScr 	$	&0.5880 &0.1492 &0.1914 &0.3095 &$(~~0,~~1,~~1,-8,-8,~~1,~~1,-4,-6)$    &550.47 &598.16 &201.58 &444.65 &0.55   &0.84\\			
				& $\SLIMLogRWepExBin 	$       &0.7778 &0.1398 &0.1778 &0.3651 &$(~~0,~~1,~~1,-6,-6,~~0,~~0,-6,-6)$    &17.15  &79.47  &744.58 &562.03 &1.00   &0.42\\			
				& \Rand  			&0.0065 &0.0023 &0.0018 &0.0035 &$(--,--,--,--,--)$\\
				& \LROnly	                &0.4494 &0.0855 &0.0846 &0.2065 &$(--,--,--,-6,-2)$\\
				& \SLIMOnly			&0.5402 &0.0971 &0.1852 &0.2742 &$(--,-3,~~0,--,--)$\\
				& \Sep		        	&0.2698 &0.1348 &0.2204 &0.2083 &$(--,~~0,~~0,-2,0)$    &953.42 &490.37 &147.12 &386.86 &0.21   &0.88\\


 	
 	






        %\hline\hline
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
        \begin{footnotesize}
        \item
        In this table, ``rec'', ``pre'', ``acc'' and ``pars'' represent
        recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
        \end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}        
  \end{threeparttable}
\end{table*}



%


==> table/performance_recall.ibk.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Recall}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & rec   & pre   & acc & avg& pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline
	\midrule								
						



				
\multirow{ 12}{*}{ \Dall } 	& $\modelInScr		$ 	&0.0287 &0.1706 &0.2534 &0.1509 &$(-3,~~1,~~0,-6,-5)$\\            	
			  	& $\modelInBin		$ 	&0.0980 &0.1662 &0.1581 &0.1408 &$(~~2,~~2,-4,-5,-7)$\\
			  	& $\modelExScr		$    	&0.1169 &0.1845 &0.2238 &0.1751 &$(~~3,-9,~~6,-7,-9)$\\
			  	& $\modelExBin		$   	&0.1253 &0.2060 &0.2657 &0.1990 &$(~~1,-\infty,~~1,-\infty,-8)$\\
%\rowcolor{gray!50}    
		          	& $\SLIMLogRWepInScr 	$      	&0.0293 &0.2168 &0.4266 &0.2242 &$(~~0,-2,-2,~~0,~~0,~~1,~~1,-4,-6)$\\
%\rowcolor{gray!50}            
			 	& $\SLIMLogRWepInBin 	$      	&0.0698 &0.2010 &0.2797 &0.1835 &$(~~0,~~0,~~0,~~0,~~0,~~1,~~1,-6,-6)$\\
%\rowcolor{gray!50}	  	
				& $\SLIMLogRWepExScr 	$ 	&0.1033 &0.1899 &0.4643 &0.2525 &$(~~0,~~0,~~0,~~0,~~0,~~1,~~1,-6,-6)$\\
%\rowcolor{gray!50}	  	
				& $\SLIMLogRWepExBin 	$ 	&0.1293 &0.2088 &0.3563 &0.2315 &$(~~0,~~1,~~1,-6,-6,~~0,~~0,-6,-6)$\\			
			  	& \Rand  			&0.0026 &0.0072 &0.0289 &0.0129 &$(--,--,--,--,--)$\\
     			  	& \LROnly	        	&0.0013 &0.0018 &0.0018 &0.0016 &$(--,--,--,-2,-1)$\\
			  	& \SLIMOnly			&0.1127 &0.1579 &0.2970 &0.1892 &$(--,-\infty,~~1,--,--)$\\
			  	& \Sep		       	  	&0.0740 &0.2011 &0.4103 &0.2285 &$(--,-2,~~2,-6,-\infty)$\\
	%\hline
	\midrule
%\rowcolor{gray!50}
\multirow{ 12}{*}{ \Dataset }	& $\modelInScr		$	&0.1514 &0.1154 &0.1208 &0.1292 &$(-3,~~1,~~0,-6,-5)$\\
%\rowcolor{gray!50}	 	
				& $\modelInBin		$	&0.4332 &0.1177 &0.1637 &0.2382 &$(~~2,~~1,-2,-6,-7)$\\
%\rowcolor{gray!50}		
				& $\modelExScr		$	&0.5709 &0.1204 &0.1467 &0.2793 &$(~~2,-7,~~4,-6,-\infty)$\\
%\rowcolor{gray!50}		
				& $\modelExBin		$	&0.7104 &0.1498 &0.1875 &0.3492 &$(~~1,-\infty,~~1,-\infty,-8)$\\
%\rowcolor{gray!50}              
				& $\SLIMLogRWepInScr 	$	&0.1620 &0.1539 &0.2683 &0.1947 &$(~~0,-2,-2,~~0,~~0,~~1,~~1,-4,-6)$\\
%\rowcolor{gray!50}              
				& $\SLIMLogRWepInBin 	$	&0.3652 &0.1349 &0.1831 &0.2277 &$(~~0,~~0,~~0,~~0,~~0,~~1,~~1,-6,-6)$\\
%\rowcolor{gray!50}              
				& $\SLIMLogRWepExScr 	$	&0.5374 &0.1269 &0.2823 &0.3155 &$(~~0,~~0,~~0,~~0,~~0,~~1,~~1,-6,-6)$\\
%\rowcolor{gray!50}              
				& $\SLIMLogRWepExBin 	$	&0.7648 &0.1584 &0.2531 &0.3921 &$(~~0,~~1,~~1,-6,-6,~~0,~~0,-6,-6)$\\    
				&\Rand  			&0.0065 &0.0023 &0.0024 &0.0037 &$(--,--,--,--,--)$\\         
				&\LROnly	                &0.0087 &0.0016 &0.0016 &0.0040 &$(--,--,--,-4,-4)$\\          
				&\SLIMOnly			&0.5404 &0.0971 &0.1852 &0.2742 &$(--,-5,~~0,--,--)$\\        
				&\Sep		                &0.3959 &0.1392 &0.2641 &0.2664 &$(--,-3,~~1,-6,-\infty)$\\   



        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'', ``acc'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_recall.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Recall}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & rec   & pre   & acc & avg& pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline
	\midrule								
						
				
\multirow{ 12}{*}{ \Dall } 	& $\modelInScr		$ 	&0.0287 &0.1706 &0.2534 &0.1509 &$(-3,~~1,~~0,-6,-5)$\\            	
			  	& $\modelInBin		$ 	&0.0980 &0.1662 &0.1581 &0.1408 &$(~~2,~~2,-4,-5,-7)$\\
			  	& $\modelExScr		$    	&0.1169 &0.1845 &0.2238 &0.1751 &$(~~3,-9,~~6,-7,-9)$\\
			  	& $\modelExBin		$   	&0.1253 &0.2060 &0.2657 &0.1990 &$(~~1,-\infty,~~1,-\infty,-8)$\\
		          	& $\SLIMLogRWepInScr 	$      	&0.0293 &0.2168 &0.2133 &0.1531 &$(~~0,-2,-2,~~0,~~0,~~1,~~1,-4,-6)$\\
			 	& $\SLIMLogRWepInBin 	$      	&0.0698 &0.2010 &0.1399 &0.1369 &$(~~0,~~0,~~0,~~0,~~0,~~1,~~1,-6,-6)$\\
				& $\SLIMLogRWepExScr 	$ 	&0.1033 &0.1899 &0.2321 &0.1751 &$(~~0,~~0,~~0,~~0,~~0,~~1,~~1,-6,-6)$\\
				& $\SLIMLogRWepExBin 	$ 	&0.1293 &0.2088 &0.1781 &0.1721 &$(~~0,~~1,~~1,-6,-6,~~0,~~0,-6,-6)$\\	
			  	& \Rand  			&0.0026 &0.0072 &0.0151 &0.0083 &$(--,--,--,--,--)$\\
     			  	& \LROnly	        	&0.0013 &0.0018 &0.0011 &0.0014 &$(--,--,--,-2,-1)$\\
			  	& \SLIMOnly			&0.1127 &0.1579 &0.2970 &0.1892 &$(--,-\infty,~~1,--,--)$\\
			  	& \Sep		       	  	&0.0791 &0.1989 &0.2279 &0.1686 &$(--,-4,~~2,-6,-4)$\\			
	%\hline
	\midrule
\multirow{ 12}{*}{ \Dataset }	& $\modelInScr		$	&0.1514 &0.1154 &0.1208 &0.1292 &$(-3,~~1,~~0,-6,-5)$\\
				& $\modelInBin		$	&0.4332 &0.1177 &0.1637 &0.2382 &$(~~2,~~1,-2,-6,-7)$\\
				& $\modelExScr		$	&0.5709 &0.1204 &0.1467 &0.2793 &$(~~2,-7,~~4,-6,-\infty)$\\
				& $\modelExBin		$	&0.7104 &0.1498 &0.1875 &0.3492 &$(~~1,-\infty,~~1,-\infty,-8)$\\
				& $\SLIMLogRWepInScr 	$	&0.1620 &0.1539 &0.1341 &0.1500 &$(~~0,-2,-2,~~0,~~0,~~1,~~1,-4,-6)$\\
				& $\SLIMLogRWepInBin 	$	&0.3652 &0.1349 &0.0915 &0.1972 &$(~~0,~~0,~~0,~~0,~~0,~~1,~~1,-6,-6)$\\
				& $\SLIMLogRWepExScr 	$	&0.5374 &0.1269 &0.1411 &0.2685 &$(~~0,~~0,~~0,~~0,~~0,~~1,~~1,-6,-6)$\\
				& $\SLIMLogRWepExBin 	$       &0.7648 &0.1584 &0.1265 &0.3499 &$(~~0,~~1,~~1,-6,-6,~~0,~~0,-6,-6)$\\	
				&\Rand  			&0.0065 &0.0023 &0.0018 &0.0035 &$(--,--,--,--,--)$\\
				&\LROnly	                &0.0087 &0.0016 &0.0012 &0.0038 &$(--,--,--,-6,-4)$\\
				&\SLIMOnly			&0.5404 &0.0971 &0.1852 &0.2742 &$(--,-5,~~0,--,--)$\\
				&\Sep		                &0.4102 &0.1379 &0.1585 &0.2355 &$(--,-\infty,-\infty,-6,-\infty)$\\




        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'', ``acc'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_recall_Rec_20.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Recall}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & \recall   &  \precision  & \accuracy & avg & pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline
	\midrule								
\multirow{ 8}{*}{ \Dall } 	 	
		          	& $\SLIMLogRWepInScr 	$    &0.0829 &0.1162 &0.1700 &0.1230 &$(~~1,-6,~~1,-2,-6)$\\   	
			 	& $\SLIMLogRWepInBin 	$    &0.0829 &0.1162 &0.1700 &0.1230 &$(~~1,-6,~~1,-2,-6)$\\   	
				& $\SLIMLogRWepExScr 	$    &0.0741 &0.1038 &0.1630 &0.1136 &$(~~0,-6,~~1,-2,-4)$\\    
				& $\SLIMLogRWepExBin 	$    &0.0741 &0.1038 &0.1630 &0.1136 &$(~~0,-6,~~1,-2,-4)$\\    
			  	& \Rand  		     &0.0021 &0.0058 &0.0139 &0.0073 &$(--,--,--,--,--)$\\
     			  	& \LROnly	             &0.0732 &0.1025 &0.1417 &0.1058 &$(--,--,--,-4,-2)$\\
			  	& \SLIMOnly		     &0.0748 &0.1047 &0.1639 &0.1145 &$(--,-4,~~2,--,--)$\\
			  	& \Sep       		     &0.0748 &0.1047 &0.1640 &0.1145 &$(--,-2,~~2,-2,~~0)$\\


	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				& $\SLIMLogRWepInScr 	$	&0.2462 &0.0442 &0.0502 &0.1135 &$(~~1,-6,~~1,-2,-6)$\\
				& $\SLIMLogRWepInBin 	$	&0.2462 &0.0442 &0.0502 &0.1135 &$(~~1,-6,~~1,-2,-6)$\\
				& $\SLIMLogRWepExScr 	$	&0.2331 &0.0419 &0.0490 &0.1080 &$(~~0,-8,~~1,-2,-4)$\\
				& $\SLIMLogRWepExBin 	$       &0.2331 &0.0419 &0.0490 &0.1080 &$(~~0,-8,~~1,-2,-4)$\\
				& \Rand  			&0.0027 &0.0010 &0.0006 &0.0014 &$(--,--,--,--,--)$\\
				& \LROnly	                &0.1674 &0.0301 &0.0184 &0.0720 &$(--,--,--,-3,-2)$\\
				& \SLIMOnly			&0.2322 &0.0417 &0.0491 &0.1077 &$(--,-1,~~1,--,--)$\\
				&\Sep           		&0.2322 &0.0417 &0.0491 &0.1077 &$(--,-1,~~1,-2,~~0)$\\


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``\recall'', ``\precision'', ``\accuracy'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_recall_Rec_20Neg.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Recall (Neg label)}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & \recall   &  \precision  & \accuracy & avg & pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline
	\midrule								
\multirow{ 8}{*}{ \Dall } 	 			                                                                         	
		          	& $\SLIMLogRWepInScr 	$  &0.0185 &0.2265 &0.1703 &0.1384 &$(,~~0,-8,~~1,-2,-6)$\\    	
			 	& $\SLIMLogRWepInBin 	$  &0.0185 &0.2265 &0.1703 &0.1384 &$(,~~0,-8,~~1,-2,-6)$\\    	
				& $\SLIMLogRWepExScr 	$  &0.0181 &0.2216 &0.1626 &0.1341 &$(,~~0,-8,~~1,-2,-2)$\\     
				& $\SLIMLogRWepExBin 	$  &0.0181 &0.2215 &0.1626 &0.1341 &$(,~~0,-8,~~1,-2,-2)$\\     
			  	& \Rand  		 &0.0020 &0.0498 &0.0139 &0.0219 &$(--,--,--,--,--)$\\       
     			  	& \LROnly	         &0.0153 &0.1873 &0.1439 &0.1155 &$(--,--,--,-2,~~0)$\\      
			  	& \SLIMOnly		 &0.0188 &0.2303 &0.1647 &0.1379 &$(--,-2,~~6,--,--)$\\      
			  	& \Sep       		 &0.0187 &0.2294 &0.1637 &0.1373 &$(--,-1,~~4,-2,~~0)$\\     


	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				& $\SLIMLogRWepInScr 	$	&0.2558 &0.0572 &0.0505 &0.1212 &$(~~0,-8,~~1,-2,-6)$\\
				& $\SLIMLogRWepInBin 	$	&0.2558 &0.0572 &0.0505 &0.1212 &$(~~0,-8,~~1,-2,-6)$\\
				& $\SLIMLogRWepExScr 	$	&0.2539 &0.0567 &0.0493 &0.1200 &$(-2,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepExBin 	$       &0.2539 &0.0567 &0.0493 &0.1200 &$(-2,-6,~~1,-2,-4)$\\	
				& \Rand  		&0.0031 &0.0014 &0.0006 &0.0017 &$(--,--,--,--,--)$\\
				& \LROnly	        &0.0347 &0.0078 &0.0181 &0.0202 &$(--,--,--,-2,~~5)$\\
				& \SLIMOnly		&0.2587 &0.0578 &0.0495 &0.1220 &$(--,-5,~~2,--,--)$\\
				&\Sep           	&0.2591 &0.0579 &0.0495 &0.1222 &$(--,-3,~~2,-2,~~0)$\\


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``\recall'', ``\precision'', ``\accuracy'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_recall_Rec_20_Top_10.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Recall Top-$10$}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & \recall   &  \precision  & \accuracy & avg & pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline

	\midrule								
\multirow{ 8}{*}{ \Dall } 	 	
		          	& $\SLIMLogRWepInScr 	$  &0.1326 &0.0929 &0.1542 &0.1266 &$(~~1,-6,~~1,-2,-4)$\\
			 	& $\SLIMLogRWepInBin 	$  &0.1326 &0.0929 &0.1541 &0.1265 &$(~~1,-6,~~1,-2,-4)$\\
				& $\SLIMLogRWepExScr 	$  &0.1214 &0.0850 &0.1467 &0.1177 &$(~~0,-8,~~1,-2,-4)$\\
				& $\SLIMLogRWepExBin 	$  &0.1214 &0.0850 &0.1467 &0.1177 &$(~~0,-8,~~1,-2,-4)$\\
			  	& \Rand  		   &0.0039 &0.0055 &0.0140 &0.0078 &$(--,--,--,--,--)$\\
     			  	& \LROnly	           &0.1191 &0.0834 &0.1458 &0.1161 &$(--,--,--,-5,-1)$\\
			  	& \SLIMOnly		   &0.1235 &0.0865 &0.1472 &0.1191 &$(--,-2,~~2,--,--)$\\
			  	& \Sep       		     &       &       &       &       &       \\









	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				& $\SLIMLogRWepInScr 	$	&0.3376 &0.0303 &0.0334 &0.1338 &$(~~1,-8,~~1,-2,-6)$\\
				& $\SLIMLogRWepInBin 	$	&0.3376 &0.0303 &0.0334 &0.1338 &$(~~1,-8,~~1,-2,-6)$\\
				& $\SLIMLogRWepExScr 	$	&0.3174 &0.0285 &0.0324 &0.1261 &$(~~0,-8,~~1,-2,-4)$\\
				& $\SLIMLogRWepExBin 	$       &0.3174 &0.0285 &0.0324 &0.1261 &$(~~0,-8,~~1,-2,-4)$\\
				& \Rand  			&0.0050 &0.0009 &0.0005 &0.0021 &$(--,--,--,--,--)$\\
				& \LROnly	                &0.2347 &0.0211 &0.0148 &0.0902 &$(--,--,--,-3,~~6)$\\
				& \SLIMOnly			&0.3156 &0.0283 &0.0334 &0.1258 &$(--,-2,~~2,--,--)$\\
				&\Sep           		&	&	&	&	&	\\


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``\recall'', ``\precision'', ``\accuracy'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_recall_Rec_20_Top_20.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Recall Top-$20$}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & \recall   &  \precision  & \accuracy & avg & pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ \\
	%\hline

	\midrule								
\multirow{ 8}{*}{ \Dall } 	 	
		          	& $\SLIMLogRWepInScr 	$   &0.2145 &0.0752 &0.1151 &0.1349 &$(~~1,~~0,~~1,-2,-2)$\\
			 	& $\SLIMLogRWepInBin 	$   &0.2146 &0.0752 &0.1149 &0.1349 &$(~~1,~~0,~~1,-2,-2)$\\
				& $\SLIMLogRWepExScr 	$   &0.1881 &0.0659 &0.1193 &0.1244 &$(~~1, -6,~~1,-2,-2)$\\
				& $\SLIMLogRWepExBin 	$   &0.1886 &0.0661 &0.1191 &0.1246 &$(~~1, -6,~~1,-2,-2)$\\
			  	& \Rand  		    &0.0080 &0.0056 &0.0142 &0.0093 &$(--,--,--,--,--)$\\
     			  	& \LROnly	            &0.1881 &0.0659 &0.1370 &0.1303 &$(--,--,--,-4,-2)$\\
			  	& \SLIMOnly		    &0.2025 &0.0709 &0.1269 &0.1334 &$(--,-1,~~6,--,--)$\\
			  	& \Sep       		    &       &       &       &       &       \\ 
















	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				
				& $\SLIMLogRWepInScr 	$	&0.4383 &0.0197 &0.0202 &0.1594 &$(~~1, -6,~~1,-2,-2)$\\
				& $\SLIMLogRWepInBin 	$	&0.4383 &0.0197 &0.0202 &0.1594 &$(~~1, -6,~~1,-2,-2)$\\
				& $\SLIMLogRWepExScr 	$	&0.4056 &0.0182 &0.0199 &0.1479 &$(~~0, -6,~~1,-2,-6)$\\
				& $\SLIMLogRWepExBin 	$       &0.4056 &0.0182 &0.0199 &0.1479 &$(~~0, -6,~~1,-2,-6)$\\
				& \Rand  			&0.0099 &0.0009 &0.0005 &0.0038 &$(--,--,--,--,--)$\\
				& \LROnly	                &0.3171 &0.0142 &0.0104 &0.1139 &$(--,--,--,-5,-2)$\\
				& \SLIMOnly			&0.4121 &0.0185 &0.0208 &0.1505 &$(--,-2,~~2,--,--)$\\
				&\Sep           	&       &       &       &       &       \\


        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``\recall'', ``\precision'', ``\accuracy'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_recall_Until_5.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Recall Until five}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
 	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
	  @{\hspace{3pt}}r@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & rec   & pre   & acc & avg& pars $(\omega, \lambda, \alpha, \gamma, \beta) 10^n$ 
			&$\text{meanN}^{+}$  &$\text{stdN}^{+}$  &$\text{meanN}^{-}$  &$\text{stdN}^{-}$  &$\text{Rec5}{\%}$ &$\text{Rec5}{\%}$\\
	%\hline
	\midrule								

\multirow{ 8 }{*}{ \Dall } 	 	
		        & $\SLIMLogRWepInScr 	$ 	&0.0300 &0.1979 &0.3853 &0.2044 &$(~~0,-2,-2,~~0,~~0,~~1,~~1,-4,-6)$    &1075.99        &374.36 &109.31 &336.01 &0.11   &0.91\\
			& $\SLIMLogRWepInBin 	$    	&0.1160 &0.1636 &0.2073 &0.1623 &$(~~0,~~0,~~0,~~0,~~0,~~1,~~1,-4,-6)$  &128.46 &274.40 &1175.19        &189.07 &0.99   &0.03\\
			& $\SLIMLogRWepExScr 	$       &0.1168 &0.1853 &0.2945 &0.1989 &$(~~0,~~0,~~0,-8,-8,~~1,~~1,-6,-6)$    &283.21 &499.99 &160.01 &399.42 &0.77   &0.87\\			
			& $\SLIMLogRWepExBin 	$       &0.1342 &0.1881 &0.2811 &0.2011 &$(~~0,~~1,~~1,-6,-6,~~0,~~0,-6,-6)$    &17.15  &79.47  &744.58 &562.03 &1.00   &0.42\\			
			& \Rand  			&0.0026 &0.0072 &0.0151 &0.0083 &$(--,--,--,--,--)$\\
     			& \LROnly	        	&0.1089 &0.1605 &0.1655 &0.1450 &$(--,--,--,-4,-2)$\\
			& \SLIMOnly			&0.1127 &0.1579 &0.2970 &0.1892 &$(--,-\infty,~~1,--,--)$\\
			& \Sep      			&0.0619 &0.1845 &0.3817 &0.2094 &$(--,-2,~~1,-2,-1)$    &855.48 &521.97 &208.52 &445.02 &0.29   &0.83\\



	%\hlinea
	\midrule
\multirow{ 8 }{*}{ \Dataset }	
				
			& $\SLIMLogRWepInScr 	$	&0.1654 &0.1401 &0.2405 &0.1820 &$(~~0,-2,-2,~~0,~~0,~~1,~~1,-4,-6)$    &1075.99        &374.36 &109.31 &336.01 &0.11   &0.91\\
			& $\SLIMLogRWepInBin 	$	&0.4965 &0.0898 &0.0870 &0.2244 &$(~~0,~~0,~~0,~~0,~~0,~~1,~~1,-4,-6)$  &128.46 &274.40 &1175.19        &189.07 &0.99   &0.03\\
			& $\SLIMLogRWepExScr 	$	&0.6002 &0.1222 &0.1767 &0.2997 &$(~~0,~~0,~~0,-8,-8,~~1,~~1,-6,-6)$    &283.21 &499.99 &160.01 &399.42 &0.77   &0.87\\			
			& $\SLIMLogRWepExBin 	$       &0.7778 &0.1398 &0.1778 &0.3651 &$(~~0,~~1,~~1,-6,-6,~~0,~~0,-6,-6)$    &17.15  &79.47  &744.58 &562.03 &1.00   &0.42\\			
			& \Rand  			&0.0065 &0.0023 &0.0018 &0.0035 &$(--,--,--,--,--)$\\
			& \LROnly	                &0.4507 &0.0852 &0.0844 &0.2068 &$(--,--,--,-4,-2)$\\
			& \SLIMOnly			&0.5404 &0.0971 &0.1852 &0.2742 &$(--,-5,~~0,--,--)$\\
			& \Sep		        	&0.3276 &0.1272 &0.2453 &0.2334 &$(--,-2,~~1,-2,-1)$    &855.48 &521.97 &208.52 &445.02 &0.29   &0.83\\


	










 	
 	
 	











        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'', ``acc'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/performance_recall_temp.tex <==
\begin{table*}[h!]
\vspace{-0mm}
  \centering
  \caption{Performance Comparison based on the Best Recall (Threshold)}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}[]{
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
	  @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule
		
	\DataPoll	&\multicolumn{1}{l}{Method} & rec   & pre   & acc & avg& pars $(\phi, \omega^{+}, \omega^{-}, \lambda^{+}, \lambda^{-}, \alpha^{+}, \alpha^{-}, \gamma, \beta) 10^n$ \\
	%\hline
	\midrule								
						
				
\multirow{ 8}{*}{ \Dall } 	
				& $\SLIMLogRWepInScr    $       &0.1252 &0.1754 &0.3065 &0.2024 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-2,-4)$\\
                                & $\SLIMLogRWepInBin    $       &0.1252 &0.1754 &0.3066 &0.2024 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-2,-4)$\\
                                & $\SLIMLogRWepExScr    $       &0.1387 &0.1943 &0.2728 &0.2019 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-6,-6)$\\
                                & $\SLIMLogRWepExBin    $       &0.1185 &0.1659 &0.2310 &0.1718 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-6,-6)$\\
                                & \Rand                         &0.0026 &0.0072 &0.0151 &0.0083 &$(--,--,--,--,--)$\\               	            
                                & \LROnly                       &0.1098 &0.1538 &0.1768 &0.1468 &$(--,--,--,-4,-2)$\\                   	        
                                & \SLIMOnly                     &0.1127 &0.1579 &0.2970 &0.1892 &$(--,-\infty,~~1,--,--)$\\                    	
                                & \Sep                          &0.1149 &0.1609 &0.2949 &0.1902 &$(--,-4,~~0,-2,~~0)$\\            	
	%\hline
	\midrule
\multirow{ 8}{*}{ \Dataset }	
				& $\SLIMLogRWepInScr    $       &0.1252 &0.1754 &0.3065 &0.2024 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-2,-4)$\\
				& $\SLIMLogRWepInBin    $       &0.1252 &0.1754 &0.3066 &0.2024 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-2,-4)$\\
				& $\SLIMLogRWepExScr    $       &0.1387 &0.1943 &0.2728 &0.2019 &$(~~0,~~1,~~1,-6,-6,~~1,~~1,-6,-6)$\\
			        & $\SLIMLogRWepExBin    $       &0.1185 &0.1659 &0.2310 &0.1718 &$(~~0,~~1,~~1,-8,-8,~~0,~~0,-6,-6)$\\
			        & \Rand                         &0.0026 &0.0072 &0.0151 &0.0083 &$(--,--,--,--,--)$\\                 
			        & \LROnly                       &0.1098 &0.1538 &0.1768 &0.1468 &$(--,--,--,-4,-2)$\\                 
			        & \SLIMOnly                     &0.1127 &0.1579 &0.2970 &0.1892 &$(--,-\infty,~~1,--,--)$\\           
				& \Sep                          &0.1149 &0.1609 &0.2949 &0.1902 &$(--,-4,~~0,-2,~~0)$\\               

        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	In this table, ``rec'', ``pre'', ``acc'' and ``pars'' represent 
	recall, precision, accuracy and parameters respectively and ``avg'' represents the average of recall, preceision and accuracy.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table*}
%


==> table/precision_top10.tex <==
        &        \multirow{2}{*}{\modelIn} &     \predScr	& 0.2497 & 0.2497 & 0.3076 \\
        &                                  &     \predBin	& 0.2497 & 0.2497 & 0.3074 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.2284 & 0.2284 & 0.2916 \\
        &                                  &     \predBin 	& 0.2284 & 0.2284 & 0.2914 \\
        &                            \Rand &            - 	& 0.0073 & 0.0148 & 0.0279 \\
        &                          \LROnly &            - 	& 0.2243 & 0.2244 & 0.2787 \\
        &                        \SLIMOnly &            - 	& 0.2323 & 0.2325 & 0.2940 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\
        &        \multirow{2}{*}{\modelIn} &     \predScr 	& 0.3464 & 0.3467 & 0.3408 \\
        &                                  &     \predBin 	& 0.3464 & 0.3467 & 0.3408 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.3257 & 0.3261 & 0.3316 \\
        &                                  &     \predBin 	& 0.3257 & 0.3261 & 0.3316 \\
        &                            \Rand &            - 	& 0.0051 & 0.0103 & 0.0051 \\
        &                          \LROnly &            - 	& 0.2408 & 0.2414 & 0.1515 \\
        &                        \SLIMOnly &            - 	& 0.3240 & 0.3238 & 0.3408 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\
        &        \multirow{2}{*}{\modelIn} &     \predScr	& 0.2497 & 0.2497 & 0.3076 \\
        &                                  &     \predBin	& 0.2497 & 0.2497 & 0.3074 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.2284 & 0.2284 & 0.2916 \\
        &                                  &     \predBin 	& 0.2284 & 0.2284 & 0.2914 \\
        &                            \Rand &            - 	& 0.0073 & 0.0148 & 0.0279 \\
        &                          \LROnly &            - 	& 0.2243 & 0.2244 & 0.2787 \\
        &                        \SLIMOnly &            - 	& 0.2323 & 0.2325 & 0.2940 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\
        &        \multirow{2}{*}{\modelIn} &     \predScr 	& 0.3464 & 0.3467 & 0.3408 \\
        &                                  &     \predBin 	& 0.3464 & 0.3467 & 0.3408 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.3257 & 0.3261 & 0.3316 \\
        &                                  &     \predBin 	& 0.3257 & 0.3261 & 0.3316 \\
        &                            \Rand &            - 	& 0.0051 & 0.0103 & 0.0051 \\
        &                          \LROnly &            - 	& 0.2408 & 0.2414 & 0.1515 \\
        &                        \SLIMOnly &            - 	& 0.3240 & 0.3238 & 0.3408 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\


==> table/precision_top20.tex <==
        &        \multirow{2}{*}{\modelIn} &     \predScr	& 0.2885 & 0.2887 & 0.2762 \\
        &                                  &     \predBin	& 0.2886 & 0.2887 & 0.2757 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.2530 & 0.2530 & 0.2862 \\
        &                                  &     \predBin 	& 0.2536 & 0.2537 & 0.2857 \\
        &                            \Rand &            - 	& 0.0108 & 0.0215 & 0.0341 \\
        &                          \LROnly &            - 	& 0.2530 & 0.2530 & 0.3287 \\
        &                        \SLIMOnly &            - 	& 0.2721 & 0.2722 & 0.3013 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\
        &        \multirow{2}{*}{\modelIn} &     \predScr 	& 0.4403 & 0.4407 & 0.4016 \\
        &                                  &     \predBin 	& 0.4403 & 0.4407 & 0.4016 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.4060 & 0.4072 & 0.3956 \\
        &                                  &     \predBin 	& 0.4060 & 0.4072 & 0.3956 \\
        &                            \Rand &            - 	& 0.0099 & 0.0201 & 0.0099 \\
        &                          \LROnly &            - 	& 0.3183 & 0.3177 & 0.2068 \\
        &                        \SLIMOnly &            - 	& 0.4140 & 0.4139 & 0.4135 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\


==> table/recall_top10.tex <==
        &        \multirow{2}{*}{\modelIn} &     \predScr	& 0.2497 & 0.2497 & 0.3076 \\
        &                                  &     \predBin	& 0.2497 & 0.2497 & 0.3074 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.2286 & 0.2284 & 0.2926 \\
        &                                  &     \predBin 	& 0.2286 & 0.2284 & 0.2926 \\
        &                            \Rand &            - 	& 0.0073 & 0.0148 & 0.0279 \\
        &                          \LROnly &            - 	& 0.2243 & 0.2241 & 0.2908 \\
        &                        \SLIMOnly &            - 	& 0.2325 & 0.2325 & 0.2936 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\
        &        \multirow{2}{*}{\modelIn} &     \predScr 	& 0.3469 & 0.3467 & 0.3419 \\
        &                                  &     \predBin 	& 0.3469 & 0.3467 & 0.3419 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.3262 & 0.3261 & 0.3316 \\
        &                                  &     \predBin 	& 0.3262 & 0.3261 & 0.3316 \\
        &                            \Rand &            - 	& 0.0051 & 0.0103 & 0.0051 \\
        &                          \LROnly &            - 	& 0.2412 & 0.2414 & 0.1515 \\
        &                        \SLIMOnly &            - 	& 0.3243 & 0.3238 & 0.3419 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\


==> table/recall_top20.tex <==
        &        \multirow{2}{*}{\modelIn} &     \predScr	& 0.2885 & 0.2887 & 0.2762 \\
        &                                  &     \predBin	& 0.2886 & 0.2887 & 0.2757 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.2530 & 0.2530 & 0.2862 \\
        &                                  &     \predBin 	& 0.2536 & 0.2537 & 0.2857 \\
        &                            \Rand &            - 	& 0.0108 & 0.0215 & 0.0341 \\
        &                          \LROnly &            - 	& 0.2530 & 0.2530 & 0.3287 \\
        &                        \SLIMOnly &            - 	& 0.2723 & 0.2722 & 0.3045 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\
        &        \multirow{2}{*}{\modelIn} &     \predScr 	& 0.4403 & 0.4407 & 0.4016 \\
        &                                  &     \predBin 	& 0.4403 & 0.4407 & 0.4016 \\
        &        \multirow{2}{*}{\modelEx} &     \predScr 	& 0.4074 & 0.4072 & 0.3956 \\
        &                                  &     \predBin 	& 0.4074 & 0.4072 & 0.3956 \\
        &                            \Rand &            - 	& 0.0099 & 0.0201 & 0.0099 \\
        &                          \LROnly &            - 	& 0.3185 & 0.3177 & 0.2068 \\
        &                        \SLIMOnly &            - 	& 0.4140 & 0.4139 & 0.4135 \\
        &                             \Sep &            - 	& 0.0000 & 0.0000 & 0.0000 \\


==> table/recommend_example_NonMyo.tex <==
\begin{table}[h!]
\vspace{-0mm}
  \centering
  \caption{Recommendation Examples NonMyopathy Recommended}
  \label{table:result_6k}
  \begin{threeparttable}
%   \begin{center}
    \begin{small}
      \begin{tabular}{
	@{\hspace{3pt}}l@{\hspace{3pt}}
        @{\hspace{3pt}}p{0.6\linewidth}@{\hspace{0pt}}
	  %@{\hspace{3pt}}l@{\hspace{3pt}}
          %@{\hspace{3pt}}l@{\hspace{3pt}}
          %@{\hspace{3pt}}l@{\hspace{3pt}}
         %
        }
        %\hline\hline
	\toprule


	Recommended drug  &Prescription \\
	%\hline
	\midrule				
acetylsalicylic acid & folic acid, \textbf{phenytoin}, alprazolam, lamotrigine, \textbf{temozolomide}, \textbf{atorvastatin}, sertraline, levetiracetam, \textbf{dexamethasone}\\
abacavir & \textbf{nelfinavir}, \textbf{tenofovir}, \textbf{zidovudine}, \textbf{ritonavir}, stavudine, \textbf{lamivudine}, \textbf{didanosine}, \textbf{zalcitabine}, lopinavir\\
alendronate & vitamin c, triamterene, valdecoxib, lisinopril, desloratadine, hydrochlorothiazide, anastrozole\\
metformin & insulin glargine, digoxin, losartan, acetylsalicylic acid, dipyridamole, glipizide, sitagliptin\\
amlodipine & bendroflumethiazide, \textbf{simvastatin}, lisinopril, \textbf{atorvastatin}\\
acetylsalicylic acid & metformin, \textbf{niacin}, clopidogrel, \textbf{rosuvastatin}\\
acetaminophen & carisoprodol, alendronate, naproxen, hydrocodone\\
salmeterol & omeprazole, loratadine, fluticasone propionate, salbutamol\\
rosiglitazone & metformin, \textbf{simvastatin}\\
risperidone & valproic acid, clozapine\\

        %\hline\hline
	\bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
	\begin{footnotesize}
	\item
	Drugs that are reported to induce myopathy are bolded.
          \par
	\end{footnotesize}
      \end{tablenotes}
    \end{small}
%   \end{center}	
  \end{threeparttable}
\end{table}
%

